Correcting inter-scan motion artefacts in quantitative R1 mapping at 7T

Purpose: Inter-scan motion is a substantial source of error in $R_1$ estimation, and can be expected to increase at 7T where $B_1$ fields are more inhomogeneous. The established correction scheme does not translate to 7T since it requires a body coil reference. Here we introduce two alternatives that outperform the established method. Since they compute relative sensitivities they do not require body coil images. Theory: The proposed methods use coil-combined magnitude images to obtain the relative coil sensitivities. The first method efficiently computes the relative sensitivities via a simple ratio; the second by fitting a more sophisticated generative model. Methods: $R_1$ maps were computed using the variable flip angle (VFA) approach. Multiple datasets were acquired at 3T and 7T, with and without motion between the acquisition of the VFA volumes. $R_1$ maps were constructed without correction, with the proposed corrections, and (at 3T) with the previously established correction scheme. Results: At 3T, the proposed methods outperform the baseline method. Inter-scan motion artefacts were also reduced at 7T. However, reproducibility only converged on that of the no motion condition if position-specific transmit field effects were also incorporated. Conclusion: The proposed methods simplify inter-scan motion correction of $R_1$ maps and are applicable at both 3T and 7T, where a body coil is typically not available. The open-source code for all methods is made publicly available.

==> 01_preambule.tex <==
%% ----------
%%   Wiley
%% ----------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% A template for Wiley article submissions.
% Developed by Overleaf. 
%
% Please note that whilst this template provides a 
% preview of the typeset manuscript for submission, it 
% will not necessarily be the final publication layout.
%
% Usage notes:
% The "blind" option will make anonymous all author, affiliation, correspondence and funding information.
% Use "num-refs" option for numerical citation and references style.
% Use "alpha-refs" option for author-year citation and references style.

% Update article type if known
% \papertype{Note}
% Include section in journal if known, otherwise delete
% \paperfield{Submitted to Magnetic Resonance in Medicine}
\graphicspath{{./figures/}}

%% ---------------
%%   Word count
%% ---------------

\newcommand{\detailtexcount}[1]{%
   \immediate\write18{texcount -merge -sum -incbib -dir #1.tex > #1.wcdetail }%
   \input{#1.wcdetail}%
}
 
\newcommand{\quickwordcount}[1]{%
   \immediate\write18{texcount -1 -sum -merge #1.tex > #1-words.sum }%
   \input{#1-words.sum} words%
}
 
\newcommand{\quickcharcount}[1]{%
   \immediate\write18{texcount -1 -sum -merge -char #1.tex > #1-chars.sum }%
   \input{#1-chars.sum} characters (not including spaces)%
}

%% ------------------
%%   Miscellaneous
%% ------------------

\usepackage{siunitx}    % SI units
\usepackage{multicol}   % multiple columns
\usepackage{caption}    % needed with multiple columns?
\usepackage{widetable}      % Tables that take the whole page width
\usepackage{booktabs}       % Nice horizontal lines for tables
\usepackage{hyperref}
\usepackage{cleveref}   % "clever references" -> allows to ref multiple equations at once
\usepackage{float}


% \newcommand*{\revised}[1]{\textcolor{red}{#1}} % annotated version
\newcommand*{\revised}[1]{#1}                  % clean version

\newenvironment{Figure}
  {\par\medskip\noindent\minipage{\linewidth}}
  {\endminipage\par\medskip}

%% -------------
%%   Math mode
%% -------------

% packages
\usepackage{amsmath}    % Base class for math
\usepackage{amssymb}    % Additional symbols
\usepackage{nicefrac}   % Nice oneliner fractions
% \usepackage{mathtools}  % Extends amsmath (multiline, extensible symbols, boxes)
\usepackage{stmaryrd}   % St Mary Road symbols: \llbracket, \rrbracket, ...

% operators
\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\argmax}{\arg\!\max}
\newcommand*{\T}{^\mathrm{T}}
\renewcommand*{\H}{^\mathrm{H}}
\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand*\Diff[1]{\mathop{}\!\mathrm{d^#1}}
\newcommand*{\dequal}{\overset{\Delta}{=}}
\newcommand*{\cequal}{\overset{c}{=}}
\newcommand*{\capprox}{\overset{c}{\approx}}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\eqdef}{=\vcentcolon}
\newcommand*{\cov}{\mathrm{cov}{}}
\newcommand*{\tr}{\mathrm{Tr}{}}
\newcommand*{\KL}{\mathrm{KL}{}}
\newcommand*{\dett}[1]{\left|#1\right|}
\renewcommand*\vec[1]{\mathbf{\boldsymbol{#1}}}
% \newcommand*\vect[1]{\boldsymbol{\mathbf{#1}}}
\newcommand*{\re}[1]{\operatorname{Re}\left\{#1\right\}}
\newcommand*{\im}[1]{\operatorname{Im}\left\{#1\right\}}


% variable names
\newcommand*{\varmean}{r}
\newcommand*{\VARMEAN}{R}
\newcommand*{\varsens}{s}
\newcommand*{\VARSENS}{S}
\newcommand*{\varlogsens}{z}
\newcommand*{\VARLOGSENS}{Z}
\newcommand*{\varmodmean}{m}
\newcommand*{\VARMODMEAN}{M}
\newcommand*{\varnoise}{\varepsilon}
\newcommand*{\VARNOISE}{E}
\newcommand*{\varkspace}{\xi}
\newcommand*{\VARKSPACE}{\Xi}
\newcommand*{\varimspace}{x}
\newcommand*{\VARIMSPACE}{X}
\newcommand*{\varnbcoil}{C}
\newcommand*{\varnbgrid}{N}
\newcommand*{\varnbobs}{K}
\newcommand*{\VARSUB}{\Phi}
\newcommand*{\VARPUSHPULL}{\Psi}

==> 02_title.tex <==
\title{Correcting inter-scan motion artefacts in quantitative $R_1$ mapping at 7T.}
% List abbreviations here, if any. Please note that it is preferred that abbreviations be defined at the first instance they appear in the text, rather than creating an abbreviations list.
% \abbrevs{ABC, a black cat; DEF, doesn't ever fret; GHI, goes home immediately.}

% Include full author names and degrees, when required by the journal.
% Use the \authfn to add symbols for additional footnotes and present addresses, if any. Usually start with 1 for notes about author contributions; then continuing with 2 etc if any author has a different present address.
\author[1,2]{Ya\"el~Balbastre}
\author[1,3]{Ali~Aghaeifar}
\author[1,4]{Nad\`ege~Corbin}
\author[1]{Mikael~Brudfors}
\author[1]{John~Ashburner}
\author[1]{Martina~F.~Callaghan}

% \contrib[\authfn{1}]{Equally contributing authors.}

% Include full affiliation details for all authors
\affil[1]{Wellcome Centre for Human Neuroimaging, UCL Queen Square Institute of Neurology, University College London, London, UK}
\affil[2]{Athinoula A. Martinos Center for Biomedical Imaging, Massachusetts General Hospital and Harvard Medical School, Boston, USA}
\affil[3]{MR Research Collaborations, Siemens Healthcare Limited, Frimley, UK}
\affil[4]{Centre de R\'esonance Magn\'etique des Syst\`emes Biologiques, UMR5536, CNRS/University Bordeaux, Bordeaux, France}

\corraddress{Martina F. Callaghan, Wellcome Centre for Human Neuroimaging, 12 Queen Square, London WC1N 3AR, UK}
\corremail{m.callaghan@ucl.ac.uk}

% \presentadd[\authfn{2}]{Department, Institution, City, State or Province, Postal Code, Country}

\fundinginfo{This work was supported by the MRC and Spinal Research Charity through the ERA-NET Neuron joint call (MR/R000050/1). The Wellcome Centre for Human Neuroimaging is supported by core funding from the Wellcome [203147/Z/16/Z]. This research was funded in whole, or in part, by the Wellcome Trust [203147/Z/16/Z]. For the purpose of open access, the author has applied a CC BY public copyright licence to any Author Accepted Manuscript version arising from this submission.}

% Include the name of the author that should appear in the running header
\runningauthor{Balbastre et al.}
